Status and implications of neutrino masses: a brief panorama

With the historic discovery of the Higgs boson our picture of particle physics would have been complete were it not for the neutrino sector and cosmology. I briefly discuss the role of neutrino masses and mixing upon gauge coupling unification, electroweak breaking and the flavor sector. Time is ripe for new discoveries such as leptonic CP violation, charged lepton flavor violation and neutrinoless double beta decay. Neutrinos could also play a role in elucidating the nature of dark matter and cosmic inflation.

==> Makefile <==
FILENAME=Proc-Neutrino-Conf-2015-new
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = Proc-Neutrino-Conf-2015-new.ps 
PDFFILE = Proc-Neutrino-Conf-2015-new.pdf

COPY = if test -r Proc-Neutrino-Conf-2015-new.toc; then cp Proc-Neutrino-Conf-2015-new.toc Proc-Neutrino-Conf-2015-new.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f Proc-Neutrino-Conf-2015-new.aux Proc-Neutrino-Conf-2015-new.log Proc-Neutrino-Conf-2015-new.dvi Proc-Neutrino-Conf-2015-new.toc Proc-Neutrino-Conf-2015-new.out Proc-Neutrino-Conf-2015-new.blg Proc-Neutrino-Conf-2015-new.mtc Proc-Neutrino-Conf-2015-new.mtc1 Proc-Neutrino-Conf-2015-new.rel Proc-Neutrino-Conf-2015-new.vrb Proc-Neutrino-Conf-2015-new.end Proc-Neutrino-Conf-2015-new.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" Proc-Neutrino-Conf-2015-new.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	Proc-Neutrino-Conf-2015-new.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)


